The MetaSUB Microbiome Core Analysis Pipeline Enables Large Scale Metagenomic Analysis

Motivation: Accurate data analysis and quality control is critical for metagenomic studies. Though many tools exist to analyze metagenomic data there is no consistent framework to integrate and run these tools across projects. Currently, computational analysis of metagenomes is time consuming, often misses potentially interesting results, and is difficult to reproduce. Further, comparison between metagenomic studies is hampered by inconsistencies in tools and databases. Results: We present the MetaSUB Core Analysis Pipeline (CAP) a comprehensive tool to analyze metagenomes and summarize the results of a project. The CAP is designed in a bottom up fashion to perform QC, preprocessing, analysis and even to build relevant databases and install necessary tools. Availability and Implementation: The CAP is available under an MIT License on GitHub at https://github.com/MetaSUB/CAP2 and on the Python Package Index. Documentation and examples are available on GitHub.

==> analysis.tex <==


